Demeter: A Parametric Model of Crop Plant Morphology from the Real World

Learning 3D parametric shape models of objects has gained popularity in vision and graphics and has showed broad utility in 3D reconstruction, generation, understanding, and simulation. While powerful models exist for humans and animals, equally expressive approaches for modeling plants are lacking. In this work, we present Demeter, a data-driven parametric model that encodes key factors of a plant morphology, including topology, shape, articulation, and deformation into a compact learned representation. Unlike previous parametric models, Demeter handles varying shape topology across various species and models three sources of shape variation: articulation, subcomponent shape variation, and non-rigid deformation. To advance crop plant modeling, we collected a large-scale, ground-truthed dataset from a soybean farm as a testbed. Experiments show that Demeter effectively synthesizes shapes, reconstructs structures, and simulates biophysical processes. Code and data is available at https://tianhang-cheng.github.io/Demeter/.

==> figure/fig2/fig2.tex <==
\begin{figure*}[t]
\vspace{-3mm}
\centering
\def\arraystretch{0.3}
\setlength{\tabcolsep}{0.5pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccc}
% &{\small Input pcd} 
&{\small ({\bf a}) + Topology ($\bGamma$)}
&{\small ({\bf b}) $\boldsymbol\Gamma$ + Articulation ($\btheta$)}
&{\small ({\bf c}) $\boldsymbol\Gamma, \boldsymbol\theta$ + Shape ($\bbeta$)}
&{\small ({\bf d}) $\boldsymbol\Gamma, \boldsymbol\theta, \bbeta$ + Deformation($\bgamma$)}

\\
% \raisebox{4mm}{\rotatebox{90}{{\small Prediction}}}
% &\includegraphics[width=0.25\linewidth]{figure/fig2/input.png}
&\includegraphics[width=0.25\linewidth]{figure/fig2/tree_v1.png}
&\includegraphics[width=0.25\linewidth]{figure/fig2/articulation_v1.png}
&\includegraphics[width=0.25\linewidth]{figure/fig2/shape_v2.png}
&\includegraphics[width=0.25\linewidth]{figure/fig2/deformation_v2.png}
\end{tabular}
}
\vspace{-16pt}
\caption{The \textbf{Demeter Model} includes four parametric components: (a) a tree-structured graph encoding plant topology with binary parameters $\bGamma$; (b) articulation parameters $\btheta$ defining each node’s relative position to its parent, using quaternions for rotation and 1D translation; (c) shape deformation $\bbeta$, representing unique leaf and stem shapes via principal component coefficients; (d) Catmull-Rom spline curves, controlled by learned linear model coefficients $\bgamma$, which deform vertices for each leaf and stem. 
% \todo{Tianhang: for all these figures on 3D mesh; I would suggest to use colors to encode each component; and use ambient occlusion and fancy shading to make the mesh looking more visually appealing; for articulation let's use a mean leaf and mean stem; but representing the orientation and location of the node; also adding a bit ambient occlusion and shadow to make the shape more 3d-ish}
}
\vspace{-12pt}
\label{fig:params}
\end{figure*}

==> figure/infer.tex <==
\begin{figure}[h!]  % [t] = place at top of page
    \centering
    % left bottom right top
    \vspace{-1pt}
    \includegraphics[width=\linewidth]{figure/inference/infer_final.pdf}
    \vspace{-2em}
    \caption{\textbf{Test-time Reconstruction Pipeline.}
    % The pipeline transforms the input images to a segmented point cloud, extracts the topology and fits part templates, and finally outputs the parametric mesh.
    }
    \label{fig:infer}
    \vspace{-12pt}
\end{figure}
